Towards More Accountable Search Engines: Online Evaluation of Representation Bias

Information availability affects people's behavior and perception of the world. Notably, people rely on search engines to satisfy their need for information. Search engines deliver results relevant to user requests usually without being or making themselves accountable for the information they deliver, which may harm people's lives and, in turn, society. This potential risk urges the development of evaluation mechanisms of bias in order to empower the user in judging the results of search engines. In this paper, we give a possible solution to measuring representation bias with respect to societal features for search engines and apply it to evaluating the gender representation bias for Google's Knowledge Graph Carousel for listing occupations.

==> notation.tex <==

Here we introduce the list of symbols and functions used in the rest of the paper.
%
\begin{longtable}{p{2cm}|p{3cm}}
    \hline
    \hline
    {\bf Symbol} & {\bf Description} \\ 
    \hline
    $\mathcal{Q}$ & The set of topics.\\
    $q$ & A topic $q \in \mathcal{Q}$.\\
    $\mathcal{R}$ & The set of runs. \\
    $r_q$ & A run $r_q \in \mathcal{R}$ for the topic $q \in \mathcal{Q}$.\\
    $\mathcal{D}$ & The collection of documents.\\
    $d$ & A document $d \in \mathcal{D}$. \\
    $\mathcal{D}_{r_q}$ & The set of documents retrieved by $r_q$.\\
    %$\mathcal{J}_q^+$ & The set of relevant documents for $q$.\\
    $\mathcal{C}$ & The set of feature values.\\
    $c$ & A feature value $c \in \mathcal{C}$.\\
    $\mathcal{F}^c$ & The set of documents marked with $c$.\\
    $\mu_q^c$ & The population mean of $c$ for $q$.\\
    \hline
    \hline
    {\bf Function} & {\bf Description} \\ 
    \hline
    %$\floor{x}$ & Rounds $x \in \mathbb{R}$ towards minus infinity (aka flooring).\\
    $[\text{Condition}]$ & Returns 1 if the condition is verified, 0 otherwise (aka Iverson bracket). \\
    %$\ceil{x}$ & Rounds $x \in \mathbb{R}$ towards plus infinity (aka ceiling).\\
    $\rho(d,r_q)$ & Returns the rank at which $d$ has been retrieved by $r_q$.\\
    %$\gamma(r,n)$ & Returns the $n$-th document retrieved by $r$.\\
    \hline
    \hline
\end{longtable}

==> related_work.tex <==

%Friedman and Nissenbaum \cite{Friedman:1996:BCS:230538.230561} classify three types of bias in information systems: 1) preexisting bias rooted in society, 2) technical bias arising from technical constraints, and 3) emergent bias arising from a change of the societal knowledge or context. 
%In this work, they argue that the quality of a system should be also evaluated in terms of freedom of bias. The bias analyzed in this paper can be the outcome of a combination of these three types of bias and we here provide the first bias measure for search engines.

%Many studies have been conducted on assessing the effect of search bias on users' perception. For example, it has been demonstrated experimentally that the ranking order of documents heavily influences users' judgment on their true relevance \cite{doi:10.1111/j.1083-6101.2007.00351.x} or their credibility \cite{IJoC636}. Kay et al.~\cite{Kay:2015:URG:2702123.2702520} demonstrated that bias in information systems alter users' perception and behavior. Kay et al.~demonstrated this by evaluating the effects of artificial bias in image search results on users' perception of prevalence of men and woman in a variety of professions.

%{\color{red}
%EXPLAIN THIS BETTER: 

INCLUDE THESE REFERENCES:
%* Measuring Fairness in Ranked Outputs, Yang&Stoyanovich, SSDBM’17:
This paper proposes various measures for quantifying the divergence between the actual and expected proportions of certain (protected) groups in ranking prefixes.
The idea is to take several well-known sta-tistical parity measures proposed in the literature [12], and makethem rank-aware by placing them within the nDCG framework [5].nDCG is commonly used for evaluating the quality of ranked listsin information retrieval, and is appropriate here because it providesa principled weighted discount mechanism. Specifically, we calcu-lateset-wise parityat a series of cut-off points in a ranking, andprogressively sum these values with a position-based discount.  
In this paper they do not care about the ratio, as far as I see here. Study Equation 5

* FA*IR: A Fair Top-k Ranking Algorithm, Zehlike et al., CIKM’17 This paper proposes a statistical test for determining whether ranking prefixes have the expected presence of certain (protected) groups.


Add These references
(see [1,2,3,4,5] as example of overview studies or links to search results for relevant work). 
"representation bias" -- a quick search on google scholar shows that this is not true (e.g., [6,7]). 

Wikipedia is not a neutral source of information [8].
Links:
%[1] https://scholar.google.com/scholar?hl=en&as_sdt=0%2C33&q=bias+in+search+engines&oq=bias+in+search+en
%[2] Baeza-Yates, Ricardo. "Data and algorithmic bias in the web." Proceedings of the 8th ACM Conference on Web Science. ACM, 2016.
%[3] Olteanu, Alexandra, et al. "Social data: Biases, methodological pitfalls, and ethical boundaries." (2016).
%[4] De-Arteaga, Maria, et al. "Bias in Bios: A Case Study of Semantic Representation Bias in a High-Stakes Setting." arXiv preprint arXiv:1901.09451 (2019).
%[5] https://scholar.google.com/scholar?hl=en&as_sdt=0%2C33&as_ylo=2018&q=bias+ranking&btnG=
%[6] Otterbacher, Jahna, Jo Bates, and Paul Clough. "Competent men and warm women: Gender stereotypes and backlash in image search results." Proceedings of the 2017 CHI Conference on Human Factors in Computing Systems. ACM, 2017.
%[7] https://scholar.google.com/scholar?as_ylo=2015&q=%22representation+bias%22&hl=en&as_sdt=0,33
%[8] https://scholar.google.com/scholar?hl=en&as_sdt=0%2C33&as_ylo=2015&q=bias+in+wikipedia&btnG=
}

%EXPERIMENTAL SECTION
%5. While the authors promise to release the code after the publication, the paper itself doesn’t contain almost any detail related to the implementation (did you actually run the ILP, what software did you use, what parameters, how did you determine the gender of the entities in the results, etc?).

%ADD IN CONCLUSION
%4. How would one go about approximating ‘mu’s for other types of attributes? To what extent does this approach generalize?
%I feel the strength of your work might be in the generalization to multiple groups, but I’d love to have seen this discussed.
